Accelerating Alternating Least Squares for Tensor Decomposition by Pairwise Perturbation

The alternating least squares algorithm for CP and Tucker decomposition is dominated in cost by the tensor contractions necessary to set up the quadratic optimization subproblems. We introduce a novel family of algorithms that uses perturbative corrections to the subproblems rather than recomputing the tensor contractions. This approximation is accurate when the factor matrices are changing little across iterations, which occurs when alternating least squares approaches convergence. We provide a theoretical analysis to bound the approximation error. Our numerical experiments demonstrate that the proposed pairwise perturbation algorithms are easy to control and converge to minima that are as good as alternating least squares. The experimental results show improvements of up to 3.1X with respect to state-of-the-art alternating least squares approaches for various model tensor problems and real datasets.

==> apx.tex <==
% \subsection{Derivation of time complexity}


% \subsection{Proof of time complexity}

% \begin{proof}
% As is shown in Theorem 6.4, in each level $l$, $\frac{(l+1)(l+2)}{2}$ tensors will be calculated. For each of them, as to the MTTKRP calculation, a tensor on level $l$, which has dimension 


% \end{proof}
% \begin{rmk}
% This is in fact a special case of coadjoint actions.
% \end{rmk}
% \begin{thm}
% \rm (Atiyah-Guillemin-Sternberg) The image of the moment map is a convex polytope. In fact, it is the convex hull of the images of the fixed points of the torus action. 
% \end{thm}
% \begin{defn}
% A fan $\Sigma \in N$ is a collection of cones $\sigma$, such that:
% \begin{itemize}
%   \item if $\sigma \in \Sigma$ and $\tau$ is a face of $\sigma$, then $\tau \in \Sigma$.
% \end{itemize}
% \end{defn}
% \begin{eg}
% $N=\Z, N_{\R}\simeq \R$, then we have the fan defined by: $\tau$=origin, $\sigm\textbf{a}_1$=positive real line, $\sigm\textbf{a}_2$=negative real line, then the dual of $\sigm\textbf{a}_1$ and $\sigm\textbf{a}_2$ correspond to the positive and negative real lines in the dual space. We have: $\C[\sigm\textbf{a}_1^{\vee}\cap M]=\C[x] $, $\C[\sigm\textbf{a}_2^{\vee}\cap M]=\C[x^{-1}] $, and $\C[\tau^{\vee}\cap M]=group \: algebra=\C[x, x^{-1}] $. Geometrically we have two inclusions of $\C^*$ into $\C$ so we get $\mathbb{P}^1$.
% \end{eg}
% \begin{ex}
% Find out what a map of fans is and show that it induces a morphism. Interprete these maps geometrically in the examples. 
% \end{ex}




% \begin{algorithm}
% \caption{ALS procedure for CP decomposition with dimension tree}\label{euclid}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
% function CP\_ALS\_DT ($\pmb{\mathcal{X}}$, $N$, $s$, $K$) \\
%     \Input{Tensor $\pmb{\mathcal{X}}$, Tensor dim $N$, size in each dim $s$, decomposition rank $K$}
%     \Output{$[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$}
% Initialize $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ \\
% Initialize HashMap$<$string,Tensor$>$ mttkrp$\_$map \\
% Initialize HashMap$<$string,string$>$ Parent  \\
% Parent $\leftarrow$ CONSTRUCT$\_$DIMENSION$\_$TREE(Parent, 1, N) \\
% \While{stopping conditions not met}
% {
%     clear mttkrp$\_$map \\
%  	\For{\texttt{$n\in [N] $}}
%     {
% 	    args $\leftarrow$ string($'a'$+n) \\
%          $\textbf{\M}_{parent}^{(n)} \leftarrow$ MTTKRP$\_$MAP$\_$DT(mttkrp$\_$map, parent, $\pmb{\mathcal{X}}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, parent[args]) \\
%          i $\leftarrow$ string($\forall s \in parent[args] \notin args$) $-'a'$ \\
%         \For{\texttt{$k\in [K] $}}
%         {
% 	     $\textbf{\M}^{(n)}(:,k)\leftarrow \textbf{\M}_{parent}^{(n)}(:,k)\times_i\textbf{A}^{(i)}(:,k)$ \\
%         }
%   $\boldsymbol{\Gamma}^{(n)}\leftarrow\textbf{S}^{(1)}\ast\cdots\ast \textbf{S}^{(n-1)}\ast \textbf{S}^{(n+1)}\ast\cdots\ast \textbf{S}^{(N)} $ \\
%     % 	\State {$ \textbf{\M}^{(n)}=\textbf{X}_{(n)}(\textbf{A}^{(1)} \odot \cdots \odot \ \textbf{A}^{(n-1)} \odot \ \textbf{A}^{(n+1)} \odot \cdots \odot \textbf{A}^{(N)})$ }
%     	 $   \textbf{A}^{(n)} \leftarrow \textbf{\M}^{(n)}(\boldsymbol{\Gamma}^{(n)})^{\dagger} $\\
%          $   \textbf{S}^{(n)} \leftarrow \textbf{A}^{(n)^T}\textbf{A}^{(n)} $      \\
%     }
%     }
%  \textbf{return} $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ \\
% \end{algorithm}

% \begin{algorithm}
% \caption{Construct the dimension tree}\label{euclid}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
% function CONSTRUCT$\_$DIMENSION$\_$TREE(Parent, start, end)
%     \Input{HashMap$<$string,string$>$ Parent, int start, int end}
%     \Output{$[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$}
%     \If{end=start} {
%      \textbf{return} \\
%     }
%     \If{end=start+1} {
%          args $\leftarrow$ string($'a'$+start) \\
%          Parent[args] $\leftarrow$ args$\_$parent \\
%          args $\leftarrow$ string($'a'$+end)  \\
% 		 Parent[args] $\leftarrow$ args$\_$parent  \\        
% 		 \textbf{return}  \\
%     }
% 	args$\_$parent $\leftarrow$ string($'a'$+start,$\cdots$,$'a'$+end) \\
%      middle $\leftarrow$ (start+end)/2 \\
%      args $\leftarrow$ string($'a'$+start,$\cdots$,$'a'$+middle) \\
%      Parent[args] $\leftarrow$ args$\_$parent \\
% 	 Parent $\leftarrow$ CONSTRUCT$\_$DIMENSION$\_$TREE(Parent, start, middle) \\
%      args $\leftarrow$ string($'a'$+middle+1,$\cdots$,$'a'$+end) \\
%      Parent[args] $\leftarrow$ args$\_$parent \\
% 	 Parent $\leftarrow$ CONSTRUCT$\_$DIMENSION$\_$TREE(Parent, middle+1, end)	 \\
%  \textbf{return} 
% \end{algorithm}

% \begin{algorithm}
% \caption{Dimension tree subprocedure for ALS CP problem}\label{euclid}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
% function MTTKRP$\_$MAP$\_$DT (mttkrp$\_$map, parent, $\pmb{\mathcal{X}}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, args) \\
%     \Input{HashMap$<$string,Tensor$>$ mttkrp$\_$map, HashMap$<$string,string$>$ parent, Tensor $\pmb{\mathcal{X}}$, Matrices $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, string args}
%     \Output{mttkrp$\_$map[args]}
%     \If{args $\in$ mttkrp$\_$map} {
%     \textbf{return} mttkrp$\_$map[args] \\
%     }
%     \If{length(args) = N/2} {
%        $[i,\cdots,j] \leftarrow$ string($\forall s \in parent[args] \notin args$) $-'a'$  \\
%         $ \textbf{\M} \leftarrow \pmb{\mathcal{X}} \times_i\textbf{A}^{(i)}$ \\
%          $ \textbf{\M}(:,k) \leftarrow \textbf{\M}(:,k) \times_{i+1}\textbf{A}^{(i+1)} (:,k)\cdots\times_j\textbf{A}^{(j)}(:,k)$ \\
%      mttkrp$\_$map[args]$\leftarrow\pmb{\mathcal{X}}$ \\
%      \textbf{return} mttkrp$\_$map[args] \\
% 	}
% 	\If{parent[args]$\notin$ mttkrp$\_$map} {
%  MTTKRP$\_$MAP$\_$DT(mttkrp$\_$map, parent, $\pmb{\mathcal{X}}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, parent[args])      \\   
%     }
%      $[i,\cdots,j] \leftarrow$ string($\forall s \in parent[args] \notin args$) $-'a'$  \\
% 	 $\textbf{\M}_{parent}$ $\leftarrow$  mttkrp$\_$map[parent[args]] \\
%       \For {$k\in[K]$} {
%         $ \textbf{\M}(:,k) \leftarrow \textbf{\M}_{parent}(:,k) \times_i\textbf{A}^{(i)}(:,k)\cdots\times_j\textbf{A}^{(j)}(:,k)$ \\
%         }
%          mttkrp$\_$map[args]$ \leftarrow \textbf{\M}$ \\
%  \textbf{return} mttkrp$\_$map[args]  \\
% \end{algorithm}

% \begin{algorithm}
% \caption{ALS procedure for Tucker decomposition with dimension tree}\label{euclid}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
% function TUCKER\_ALS \\
% \Input{Tensor $V$, \\ Tensor dim $N$, \\ size in each dim $s$, \\ decomposition rank $K$}
% \Output{$[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$}
%  Initialize $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ \\
%  Initialize HashMap$<$string,Tensor$>$ ttmc$\_$map \\
%  Initialize HashMap$<$string,string$>$ parent \\
%  Parent $\leftarrow$ CONSTRUCT$\_$DIMENSION$\_$TREE(Parent, 1, N)  \\
% \While{stopping conditions not met} {
%     {clear ttmc$\_$map}  \\
% 	\For{{$n\in [N] $}} {
%      args $\leftarrow$ string($'a'$+n) \\
%      $\pmb{\mathcal{Y}}_{parent} \leftarrow$ TTMC$\_$MAP$\_$DT(ttmc$\_$map, parent, $\pmb{\mathcal{X}}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, parent[args]) \\
%       i $\leftarrow$ string($\forall s \in parent[args] \notin args$) $-'a'$  \\
% 	  $\pmb{\mathcal{Y}}\leftarrow \pmb{\mathcal{Y}}_{parent}\times_i\textbf{A}^{(i)}$ \\
%     {$   \textbf{A}^{(n)} \leftarrow $ K leading left singular vectors of $\textbf{Y}_{(n)} $}  \\
% 	}
%   {$\pmb{\mathcal{G}}\leftarrow\pmb{\mathcal{X}}\times_1\textbf{A}^{(1)T}\cdots\times_{N}\textbf{A}^{(N)T}$} \\

% }
%  \textbf{return} $[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ \\
% \end{algorithm}

% \begin{algorithm}
% \caption{Dimension tree subprocedure for ALS Tucker problem}\label{euclid}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
% function  TTMC$\_$MAP$\_$DT \\
% \Input{HashMap$<$string,Tensor$>$ ttmc$\_$map, HashMap$<$string,string$>$ parent, Tensor $\pmb{\mathcal{X}}$, Matrices $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, string args}
% \Output{$[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$}
%  Initialize $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ \\
%     \If{args = string($'a',\cdots,'a'+N$)} {
%      ttmc$\_$map[args]$\leftarrow\pmb{\mathcal{X}}$ \\
%      \textbf{return} ttmc$\_$map[args] \\
%     }
%     \If{args $\in$ ttmc$\_$map} {
%      \textbf{return} ttmc$\_$map[args] \\
%     }
%     \If{parent[args]$\notin$ ttmc$\_$map}  {
%  TTMC$\_$MAP$\_$DT(ttmc$\_$map, parent, $\pmb{\mathcal{X}}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, parent[args])        \\ 
%     }
%     $[i,\cdots,j] \leftarrow$ string($\forall s \in parent[args] \notin args$) $-'a'$   \\
%  $\pmb{\mathcal{M}}_{parent}$ $\leftarrow$  ttmc$\_$map[parent[args]]   \\
%       $ \pmb{\mathcal{M}} \leftarrow \pmb{\mathcal{M}}_{parent} \times_i\textbf{A}^{(i)}\cdots\times_j\textbf{A}^{(j)}$  \\
%       mttkrp$\_$map[args]$ \leftarrow \pmb{\mathcal{M}}$ \\
%  \textbf{return} mttkrp$\_$map[args]  \\
% \end{algorithm}


==> cond.tex <==
Our error analysis makes use of the conditioning of the product between a tensor and vectors along all except one mode.
This conditioning analysis is not directly related to the conditioning of CP decomposition~\cite{de2008tensor,vannieuwenhoven2017condition,breiding2018condition}.

\subsection{Tensor Condition Number}

We introduce a notion of a tensor condition number that corresponds to the conditioning of the multilinear vector-valued functions, 
$\fvcr{g}^{(n)}_{\tsr{T}} : \otimes_{i=1,i\neq n}^{N} \mathbb{R}^{s_{i}} \to \mathbb{R}^{s_n}$ associated with the product of the tensor with vectors along all except the $n$th mode,
\[\fvcr{g}^{(n)}_{\tsr{T}}(\vcr{x}_1,\ldots,\vcr{x}_{n-1},\vcr{x}_{n+1},\ldots, \vcr{x}_{N}) = \mat{T}_{(n)} \bigcirc_{i=1,i\neq n}^N\vcr{x}_i.\]
We consider the conditioning of a tensor for a given set of $N-1$ vectors based on the sensitivity of any $\fvcr{g}^{(n)}_{\tsr{T}}$ to the worst case perturbation of any input $\vcr{x}_m$ for $m\neq n$,
\begin{align*}
%\kappa_{\tsr{T}}(\vcr{x}_1,\ldots, \vcr{x}_n) &{=} \max_{n\in \{1,\ldots, N\}} \kappa_{\fvcr{g}^{(n)}_{\tsr{T}}}(\vcr{x}_1,\ldots,\vcr{x}_{n-1},\vcr{x}_{n+1},\ldots, \vcr{x}_{N}), \quad \text{where} \\
\kappa(\fvcr{g}^{(n)}_{\tsr{T}},\vcr{y}_1,\ldots,\vcr{y}_{N-1}) &= \max_{m\in \{1,\ldots, N-1\}} \max_{d\vcr{y}\neq \vcr 0} \frac{||\fvcr{g}^{(n)}_{\tsr{T}}(\vcr{y}_1,\ldots,\vcr{y}_{m}{+}d\vcr{y},\ldots, \vcr{y}_{N-1})||_2 ||\vcr{y}_m||_2}{||\fvcr{g}^{(n)}_{\tsr{T}}(\vcr{y}_1,\ldots, \vcr{y}_{N-1})||_2 ||d\vcr{y}||_2}.
\end{align*}
%In particular, each equidimensional order $N$ tensor $\tsr{T}$ can be associated with a vector-valued function
%\[\fvcr{g}_{\tsr{T}}(\vcr{x}_1,\ldots, \vcr{x}_{N-1}) = \mat{T}_{(1)} (\vcr{x}_1 \circ \cdots  \circ \vcr{x}_{N-1}).\]
The magnitude of the perturbation is not relevant, since each $\fvcr{g}^{(n)}$ is linear with respect to one of its inputs.
In particular, the matrix defining the linear operator acting on the $m$th input vector for $\fvcr{g}^{(n)}$ (with all other inputs fixed) corresponds to the pairwise perturbation operator arising for a rank-1 CP or Tucker decomposition (Definitions~\ref{def:tensors-cp} and~\ref{def:tensors-tucker}), given by the matrix,
$$\tsr{M}^{(i_m,i_n)} = \tsr{T}_{(m,n)} \bigcirc_{i=1,i\neq m,n}^N \vcr{x}_i.$$
Consequently, the tensor condition number is the highest condition number of any of the pairwise perturbation operator matrices for a given set of vectors $\vcr{x}_1,\ldots, \vcr{x}_n$,
\[\kappa_{\tsr{T}}(\vcr{x}_1,\ldots, \vcr{x}_n) = \max_{m,n\in\{1,\ldots N\}, m\neq n} \kappa\big(\mat{M}^{(i_m,i_n)}\big).\]




==> cost.tex <==
In this section we describe dimension-tree pairwise perturbation algorithms and provide a detailed cost analysis.

 \begin{algorithm}
\caption{\textbf{CP\_ALS\_PP}: Pairwise perturbation algorithm for ALS-CP}\label{cpalspp}
\begin{algorithmic}[1]
\footnotesize
\STATE{\textbf{Input: }Tensor $\tsr{V}$, Tensor dimension $N$, Sizes in each dimension \{$s_1, \cdots, s_N$\}, Decomposition rank $K$, Stopping criteria $\varepsilon$, Stopping criteria for pairwise perturbation subprocedure $\varepsilon_{pp}$}
\STATE{Initialize $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ }
\STATE{$\tree{T}\leftarrow$ Construct$\_$PP$\_$Tree(Parent, args)   \COMMENT{\fontfamily{qcr}\selectfont\footnotesize Construct the tree based on Definition~\ref{def:pptree}}}
\STATE{Initialize \textbf{Map}$<$TreeNode, Tensor$>$  \COMMENT{\fontfamily{qcr}\selectfont\footnotesize Map of TreeNodes to Tensors}}
\WHILE{$\sum_{i=1}^{N}{\fnrm{\mat{G}^{(i)}}}>\varepsilon$}
\STATE{$~[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$$~\leftarrow$ CP$\_$ALS$\_$DT$\_$Sub($~\tsr{V}$, N, K, $~\varepsilon_{pp}~$,$~[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]~$) \COMMENT{\fontfamily{qcr}\selectfont\footnotesize Running ALS-CP based on the dimension tree based algorithm. The stopping criteria is the perturbation magnitude $d\mat{A}^{(i)}$ are all less that $\varepsilon_{pp}$. }}

\STATE{$~[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]~\leftarrow$ CP$\_$ALS$\_$PP$\_$Sub($\tsr{V}$,N,K,$\tree{T}$,\textbf{~Map~},$\varepsilon_{pp},[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$)}

\ENDWHILE
\RETURN $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$
\end{algorithmic}
\end{algorithm}

\subsection{CP-ALS}
\label{sec:cost-cp}
The detailed algorithm for the CP decomposition with pairwise perturbation is in Algorithm~\ref{cpalspp}. Below we define the pairwise construction tree that is used in the pairwise perturbation algorithm for intermediate tensor construction, and we prove in Theorem~\ref{thm:cost} that it is asymptotically faster than the dimension tree based CP algorithm~\cite{kaya2016parallel,ballard2017communication}.
\begin{defn}
\label{def:pptree}
A \textbf{pairwise perturbation construction tree} $\tree{T}$ for N dimensions is a rooted tree with $N(N-1)/2$ leaf nodes. The \textbf{root} of the tree is denoted by $Root(\tree{T})$, and the \textbf{leaf} nodes are denoted by $Leaves(\tree{T})$. Each $t\in \tree{T}$ is associated with a \textbf{mode set} $\mu(t) \subseteq \mathbb{N}_N$, and the parent node denotes $Parent(t)$. The tree satisfies the following properties:
\begin{itemize}
  \item $\mu(Root({\tree{T}})) = \emptyset$.
  \item For $\forall i,j\in[1,N]$, $i\neq j$, the leaf node $
  \tree{T}_{(i,j)}\in Leaves(\tree{T})$ and $\mu({\tree{T}_{(i,j)}}) = \mathbb{N}_N\setminus\{i,j\}$.
  \item Each tree level $l\in[1,N-2]$, includes the tree nodes $\tree{T}_{(i,j,l+3,l+4,\ldots, N)}, \forall i,j\in[1,l+2], i\neq j$.
  \item The parent of each node $\tree{T}_{(i,j,l+3,l+4,\ldots, N)}$ is $\tree{T}_{(s,t,v,l+3,l+4,\ldots, N)}$ where \\ $\{s,t,v\}=\{i,j\}\cup \{\max_{w\in \{l,\ldots, l+2\}\setminus\{i,j\}}(w)\}$ and $s<t<v$.
\end{itemize}
\end{defn}
 
\begin{algorithm}
\caption{\textbf{CP\_ALS\_PP}: Pairwise perturbation algorithm for CP-ALS}\label{cpalspp}
\begin{algorithmic}[1]
\footnotesize
\STATE{\textbf{Input:} Tensor $\tsr{V}$, Tensor dimension $N$, Decomposition rank $K$, Pairwise perturbation construction tree $\tree{T}$, Map of TreeNode and Tensor \textbf{Map}, Tolerance $\varepsilon$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ }
%\STATE{clear \textbf{Map}} 
\FOR{$i\in [1,N] $} 
\STATE{$   \textbf{A}_p^{(n)} \leftarrow \textbf{A}^{(n)} $}  
\STATE{$   \textbf{dA}^{(n)} \leftarrow\textbf{O} $}
\ENDFOR
\FOR{\texttt{$i,j\in [1,N], i\neq j $}} 
\STATE{
    get TreeNode t such that $\mu(t) = \mathbb{N}_N\setminus\{i,j\}$}
% 	 args $\leftarrow$ string($'a',\cdots,'a'+i-1,'a'+i+1,\cdots,'a'+j-1,'a'+j+1,\cdots,'a'+N$) \\
     \STATE{$\pmb{\mathcal{M}}_p^{(i,j)}\leftarrow$ Tree$\_$Map$\_$PP(\textbf{Map}, $\tree{T}$, $\tsr{X}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, t) }
\ENDFOR
\FOR{{$i\in [1,N] $}} 
     \STATE{$\mat{M}_p^{(i)}\leftarrow \mat{M}_{p(j)}^{(i,j)}\mat{A}^{(j)}$ }
\ENDFOR 
\WHILE{$\forall ~i \in [1,N], {\frac{\fnrm{d\mat{A}^{(i)}}}{\fnrm{d\mat{A}^{(i)}}}}<\varepsilon$}
\FOR{\texttt{$n\in [1,N] $}}
  \STATE{$\boldsymbol{\Gamma}^{(n)}\leftarrow\textbf{S}^{(1)}\ast\cdots\ast \textbf{S}^{(n-1)}\ast \textbf{S}^{(n+1)}\ast\cdots\ast \textbf{S}^{(N)} $} 
    \FOR{$k\in [1,K]$} 
    	 \STATE{$ \textbf{\M}^{(n)}(:,k)\leftarrow\textbf{\M}_p^{(n)}(:,k) + \sum_{i=1,i\neq n}^{N}\textbf{\M}_p^{(i,n)}\times_i d\textbf{A}^{(i)}(:,k)$ } 
    \ENDFOR
    	 \STATE{$   \textbf{A}^{(n)} \leftarrow \textbf{\M}^{(n)}(\boldsymbol{\Gamma}^{(n)})^{\dagger} $}   	
         \STATE{$   \textbf{S}^{(n)} \leftarrow \textbf{A}^{(n)^T}\textbf{A}^{(n)} $}
    	 \STATE{$   d\textbf{A}^{(n)}\leftarrow \textbf{A}^{(n)}-\textbf{A}_p^{(n)} $}
\ENDFOR
\ENDWHILE

 \RETURN $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ \\
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\textbf{Tree$\_$Map$\_$PP}: Construction procedure for PP dimension tree map}\label{euclid}
\begin{algorithmic}[1]
\footnotesize
\STATE{\textbf{Input:} Tensor $\pmb{\mathcal{X}}$, Map of TreeNode and Tensor \textbf{Map}, Pairwise perturbation construction tree $\tree{T}$,  $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, TreeNode t}
\IF{t $\in$ \textbf{Map}} 
    \RETURN \textbf{Map}[t]
\ENDIF
    \STATE{$i \leftarrow$ max number in $\mu(t)$}
    \IF{size($\mu(t)$)=1   
    \COMMENT{{\fontfamily{qcr}\selectfont\footnotesize It's the last matrix to contract}} }
         \STATE{$ \tsr{M} \leftarrow \pmb{\mathcal{X}} \times_i\textbf{A}^{(i)}$}
         \STATE{\textbf{Map}[t]$ \leftarrow \tsr{M}$}
 \RETURN \textbf{Map}[t]
    \ENDIF
    \IF{Parent[t]$\notin$ \textbf{Map}} {
 \STATE{Tree$\_$Map$\_$PP(\textbf{Map}, $\tree{T}$, $\pmb{\mathcal{X}}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, Parent[t])      }  
    }
    \ENDIF
	\STATE{$\tsr{M}_{parent}$ $\leftarrow$  \textbf{Map}[Parent[t]]}
    \FOR {$k\in[1,K]$} 
         \STATE{$ \tsr{M}(:,k) \leftarrow \tsr{M}_{parent}(:,k) \times_i\textbf{A}^{(i)}(:,k)$ }
    \ENDFOR
        \STATE{ \textbf{Map}[t]$ \leftarrow \tsr{M}$ }
 \RETURN \textbf{Map}[t] 
\end{algorithmic}
\end{algorithm}




\begin{lemma}
\label{lemma:cost}
\rm To get $\pmb{\mathcal{M}}^{(i,j)}$ with $ \forall i\neq j$, $i,j\in [1,N]$, $\frac{(l+1)(l+2)}{2}$ tensors will be calculated on each level $l\in[1,N-2]$ with $\textbf{Algorithm~\ref{cpalspp}}$.
\end{lemma}
\begin{proof}
Based on Definition~\ref{def:tensors-cp}, we seek 
$\tsr{M}^{(i,j)}$ with $ \forall i\neq j$, $i,j\in [1,N]$. These are the tensors in $\mat{T}_{N-2}$. In Algorithm~\ref{cpalspp}, on each level $l$, all the possible $\tsr{M}^{(i_1,i_2,\cdots,i_{N-l})}$ are calculated, where $\{i_1,i_2,\cdots,i_{N-l}\}=\mathbb{N}_N\setminus\{j_1,j_2,\cdots,j_l\}$, and $\{j_1,j_2,\cdots,j_l\}$ are the first $l$ indexes for the ${l+2 \choose 2}$ tensors in $\mat{T}_{N-2}$.
% There're ${l+2 \choose 2}$ different tensors on each level, which is $\frac{(l+1)(l+2)}{2}$.
\end{proof}
Based on the above analysis, the complexity of approximated MTTKRP calculations in Algorithm~\ref{cpalspp} for every step is
\begin{align*} 
    %\begin{array}{l}
       T&=\underbrace{\frac{s^NR}{I}\sum_{l=2}^{N-1}l(l+1)s^{-(l-2)}}_\text{come from $\tsr{M}^{(i,j)}_p$ calculations}\text{         }+\underbrace{2Ns^2R}_\text{come from $\mat{M}^{(i)}$ calculations} \\
    %\end{array}   
&=\frac{2}{I}\bigg{(}3s^NR+6s^{N-1}R+10s^{N-2}R+\frac{s^NR}{2}\sum_{l=5}^Nl(l+1)s^{-(l-2)}\bigg{)}+2Ns^2R \\
&\leq\frac{2}{I}\bigg{(}3s^NR+6s^{N-1}R+10s^{N-2}R+\frac{s^NR}{2}\int_{l=4}^Nl(l+1)s^{-(l-2)}dl\bigg{)}+2Ns^2R \\
&\leq\frac{2}{I}\bigg{(}3s^NR+6s^{N-1}R+25.5s^{N-2}R\bigg{)}+2Ns^2R.
\end{align*}
When $I\geq 10$, $s\geq 20$ and $N\geq 4$, considering that $T > 4s^NR$ with the regular ALS dimension tree algorithm, the pairwise perturbation method is at least 6 times faster. 

\subsection{Tucker-ALS}
\label{sec:cost-tucker}
%\begin{algorithm}
%\caption{\textbf{Tucker\_ALS\_PP}: Pairwise perturbation algorithm for ALS-Tucker}\label{tuckeralspp}
%\begin{algorithmic}[1]
%\footnotesize
%\STATE{\textbf{Input: }Tensor $\tsr{V}$, Tensor dimension $N$, Sizes in each dimension \{$s_1, \cdots, s_N$\}, Decomposition ranks $\{R_1,\cdots,R_N\}$, 
%Stopping criteria $\varepsilon$, Stopping criteria for pairwise perturbation subprocedure $\varepsilon_{pp}$
%}
%\STATE{Initialize $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ }
%\STATE{$\tree{T}\leftarrow$ Construct$\_$PP$\_$Tree(Parent, args)   \COMMENT{\fontfamily{qcr}\selectfont\footnotesize Construct the tree based on Definition~\ref{def:pptree}}}
%\STATE{ Initialize \textbf{Map}$<$TreeNode, Tensor$>$  \COMMENT{\fontfamily{qcr}\selectfont\footnotesize It maps any TreeNode to a Tensor and stores it}}
%\STATE{$t \leftarrow 0$}
%\WHILE{$|\fnrm{\tsr{G}_t}-\fnrm{\tsr{G}_{t-1}}|>\varepsilon$} 
%\STATE{$t\leftarrow t+1$ }
%\STATE{$[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]\leftarrow$ Tucker$\_$ALS$\_$DT$\_$Sub($\tsr{V}$,N,K, $\varepsilon_{pp}$,$[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$) \COMMENT{\fontfamily{qcr}\selectfont\footnotesize Running ALS-CP based on the dimension tree based algorithm. The stopping criteria is the perturbation magnitude $d\mat{A}^{(i)}$ are all less that $\varepsilon_{pp}$.}}
%\STATE{
%$[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]\leftarrow$ Tucker$\_$ALS$\_$PP$\_$Sub($\tsr{V}$,N,K,$\tree{T}$,$\textbf{Map}$,$[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$)}
%\ENDWHILE
% \RETURN $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ 
%\end{algorithmic}
%\end{algorithm}

\begin{algorithm}
\caption{\textbf{Tucker\_ALS\_PP}: Pairwise perturbation algorithm for Tucker-ALS}\label{tuckerpp}
\begin{algorithmic}[1]
\footnotesize
\STATE{\textbf{Input:} Tensor $\tsr{X}$, Tensor dimension $N$, Decomposition ranks $\{R_1,\cdots,R_N\}$, Pairwise perturbation construction tree $\tree{T}$, Map of TreeNodes to Tensor, Tolerance $\varepsilon$, $[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$
}
%\STATE{clear \textbf{Map}}
	\FOR{{$i\in [1,N] $}} {
    	\STATE{$   \textbf{A}_p^{(n)} \leftarrow \textbf{A}^{(n)} $}  
    	\STATE{$   \textbf{dA}^{(n)} \leftarrow\textbf{O} $}
	
    }\ENDFOR
	\FOR{\texttt{$i,j\in [1,N], i\neq j $}} {
    \STATE{get TreeNode t such that $\mu(t) = \mathbb{N}_N\setminus\{i,j\}$}
     \STATE{$\pmb{\mathcal{Y}}_p^{(i,j)}\leftarrow$ Tree$\_$Map$\_$PP(\textbf{Map}, $\tree{T}$, $\tsr{X}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, t) }
	}\ENDFOR
	\FOR{{$i\in [1,N] $}} {
     \STATE{$\tsr{Y}_p^{(i)}\leftarrow \tsr{Y}_{p}^{(i,j)}\times_j\mat{A}^{(j)}$ }
	}\ENDFOR     
\WHILE{$\forall ~i \in [1,N], {\fnrm{d\mat{A}^{(i)}}}<\varepsilon$}{	\FOR{\texttt{$n\in [N] $}} {
     \STATE{$ \pmb{\mathcal{Y}}\leftarrow\pmb{\mathcal{Y}}_p^{(n)} + \sum_{i=1,i\neq n}^{N}\pmb{\mathcal{Y}}_p^{(i,n)}\times_i d\textbf{A}^{(i)}$ }
     \STATE{$   \textbf{A}^{(n)} \leftarrow R_n$ leading left singular vectors of $\textbf{Y}_{(n)}$}
     \STATE{$   d\textbf{A}^{(n)} \leftarrow\textbf{A}^{(n)}-\textbf{A}_p^{(n)} $}
	}
	\ENDFOR
\STATE{$\pmb{\mathcal{G}}\leftarrow\pmb{\mathcal{X}}\times_1\textbf{A}^{(1)T}\cdots\times_{N}\textbf{A}^{(N)T}$}
	}\ENDWHILE

 \RETURN $[\![\pmb{\mathcal{G}}; \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$ 
\end{algorithmic}
\end{algorithm}

The detailed algorithm for the Tucker decomposition with pairwise perturbation is in Algorithm~\ref{tuckerpp}. Definition~\ref{def:pptree} that applied to CP decomposition is also applicable to Tucker decomposition. 
%Using Theorem~\ref{thm:costtucker}, we also prove that our algorithm is much faster than the dimension tree based Tucker algorithm. 
%\begin{thm}
%\label{thm:costtucker}
%\rm To get $\tsr{Y}^{(i,j)}$ with $ \forall i\neq j$, $i,j\in [1,N]$, $\frac{(l+1)(l+2)}{2}$ tensors will be calculated on each level $l\in[1,N-2]$ with $\textbf{Algorithm~\ref{tuckerpp}}$.
%\end{thm}
%\begin{proof}
%Proof to the Theorem is the same as Proof to Theorem~\ref{thm:cost}.
%\end{proof}
Based on the above analysis, the complexity of approximated TTMc calculations in Algorithm~\ref{tuckerpp} for every step is
\begin{align*} 
    %\begin{array}{l}
       T&=\underbrace{\frac{s^NR}{I}\sum_{l=2}^{N-1}l(l+1)(\frac{R}{s})^{(l-2)}}_\text{come from $\tsr{Y}^{(i,j)}_p$ calculations}\text{         }+\underbrace{2Ns^2R^{N-1}}_\text{come from $\tsr{Y}^{(i)}$ calculations} \\
    %\end{array}   
&=\frac{2}{I}\bigg{(}3s^NR+6s^{N-1}R^2+10s^{N-2}R^3+\frac{s^NR}{2}\sum_{l=5}^Nl(l+1)(\frac{R}{s})^{(l-2)}\bigg{)}+2Ns^2R^{N-1} \\
&\leq\frac{2}{I}\bigg{(}3s^NR+6s^{N-1}R^2+10s^{N-2}R^3+\frac{s^NR}{2}\int_{l=4}^Nl(l+1)(\frac{R}{s})^{(l-2)}dl\bigg{)}+2Ns^2R^{N-1} \\
&\leq\frac{2}{I}\bigg{(}3s^NR+6s^{N-1}R^2+25.5s^{N-2}R^3\bigg{)}+2Ns^2R^{N-1}.
\end{align*}
When $I\geq 10$, $\frac{s}{R}\geq 5$ and $N\geq 4$, considering that $T > 4s^NR$ with dimension tree algorithm, the pairwise perturbation method is at least 3 times faster.

We note that our cost analysis for MTTKRP and TTMc is limited to dense tensors. For decomposition of sparse tensors, the contraction between the input tensor and the first matrix will cost less operations and will be more efficient. Therefore, the potential speed-up of pairwise perturbation for sparse tensors is likely lesser. 




\begin{algorithm}
\caption{\textbf{Ttmc$\_$Map$\_$PP}: Subprocedure for building Tucker-PP map}\label{alg:mapttmc}
\begin{algorithmic}[1]
\footnotesize
\STATE{\textbf{Input: }Map of TreeNode and Tensor \textbf{Map}, Pairwise perturbation construction tree $\tree{T}$, Tensor $\pmb{\mathcal{X}}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, TreeNode t}
    \IF{t $\in$ \textbf{Map}} {
     \RETURN \textbf{Map}[t]
    }\ENDIF
     \STATE{$i \leftarrow$ max number in $\mu(t)$ }
    \IF{size($\mu(t)$)=1  \COMMENT{{\fontfamily{qcr}\selectfont\footnotesize It's the last matrix to contract}}} {  
         \STATE{$ \tsr{Y} \leftarrow \pmb{\mathcal{X}} \times_i\textbf{A}^{(i)}$ }
         \STATE{\textbf{Map}[t]$ \leftarrow \tsr{Y}$ }
 \RETURN \textbf{Map}[t]
}\ENDIF
    \IF{Parent[t]$\notin$ \textbf{Map}} {
 \STATE{Ttmc$\_$Map$\_$PP(\textbf{Map}, $\tree{T}$, $\pmb{\mathcal{X}}$, $[\![ \textbf{A}^{(1)}, \cdots , \textbf{A}^{(N)} ]\!]$, Parent[t])       }
    }\ENDIF
		 \STATE{$\tsr{Y}_{parent}$ $\leftarrow$  \textbf{Map}[Parent[t]] }
         \STATE{$ \tsr{Y} \leftarrow \tsr{Y}_{parent} \times_i\textbf{A}^{(i)}$ }
         \STATE{\textbf{Map}[t]$ \leftarrow \tsr{Y}$ }
 \RETURN \textbf{Map}[t]  
\end{algorithmic}
\end{algorithm}

